Automating Urban Soundscape Enhancements with AI: In-situ Assessment of Quality and Restorativeness in Traffic-Exposed Residential Areas

Formalized in ISO 12913, the "soundscape" approach is a paradigmatic shift towards perception-based urban sound management, aiming to alleviate the substantial socioeconomic costs of noise pollution to advance the United Nations Sustainable Development Goals. Focusing on traffic-exposed outdoor residential sites, we implemented an automatic masker selection system (AMSS) utilizing natural sounds to mask (or augment) traffic soundscapes. We employed a pre-trained AI model to automatically select the optimal masker and adjust its playback level, adapting to changes over time in the ambient environment to maximize "Pleasantness", a perceptual dimension of soundscape quality in ISO 12913. Our validation study involving ($N=68$) residents revealed a significant 14.6 % enhancement in "Pleasantness" after intervention, correlating with increased restorativeness and positive affect. Perceptual enhancements at the traffic-exposed site matched those at a quieter control site with 6 dB(A) lower $L_\text{A,eq}$ and road traffic noise dominance, affirming the efficacy of AMSS as a soundscape intervention, while streamlining the labour-intensive assessment of "Pleasantness" with probabilistic AI prediction.

==> body/01introduction_old_.tex <==
\section{Introduction}
\label{sec:Introduction}

\subsection{Background and Motivation}

The emergence of increased public health risks and burden of disease from environmental noise exposure has led to the recent reduction in recommended noise limits by the World Health Organisation \citep{WorldHealthOrganizationRegionalOfficeforEurope2018}. This pervasiveness of noise, especially in urban areas, and its myriad of associated severe health risks is akin to being exposed to a "new secondhand smoke" \citep{Fink2019}. Noise exposure is the most severe in urbanised areas \citep{Basu2021}, especially in high-density, high-rise topographies \citep{Yuan2019ExaminingChina}. The continued adoption of remote work post-pandemic has brought about renewed impetus and urgency for noise abatement in now dual-function dwellings (i.e. for work and rest). 

Environmental noise mitigation is trifold by nature and is most effective at the source, followed by along the propagation path, and finally at the receivers' end \citep{Lam2021,EuropeanEnvironmentAgency2020}. Land-scarce, high-density and high-rise urban areas, however, reduce the feasibility and efficacy of traditional noise management measures along the propagation path (e.g. low high-rise efficacy of noise barriers, unavailable land for building setback guidelines) and at the source (e.g. limited airspace) \citep{Lam2021,Bin2019}. Hence, despite the reduced efficacy, mitigation at the receivers' end (e.g., windows) plays an increasingly important role in the overall noise management strategy. 

However, the path towards sustainable urban development (i.e. United National Sustainable Development Goals \citep{UnitedNationsGeneralAssembly2015}) has imposed additional challenges to effective noise mitigation in dwellings. The rapid adoption of natural ventilation (NV) in buildings to safeguard public health \citep{Nathalie2011HealthSector,Morawska2020HowMinimised}, and reduce building energy consumption \citep{Tong2016,Cao2016BuildingDecade,Spandagos2017EquivalentCities} has imposed a forced trade-off between NV and noise insulation with regards to façade openings (i.e. windows). Moreover, access to outside sounds as a result of natural ventilation was also found to increase content [\citet{Torresin2020IndoorBuildings}; i.e. related and analogous to arousal and eventfulness in the circumplex models of affect \citep{Russell1980AAffect.}, and perceived affective quality \citep{InternationalOrganizationforStandardization2019}, respectively], and when coupled with increased comfort in the presence of outdoor natural sounds, forms an engaging environment for both work from home and relaxation \citep{Torresin2022}. Therefore, noise mitigation strategies that preserve NV are essential to alleviating this forced trade-off of increased noise ingress with the opening of windows for NV. 

Of the NV-preserving noise control measures for façade openings \citep{Tang2017,Torresin2019a}, active noise control (ANC) strategies have demonstrated significant noise reduction performance with minimal impact on airflow \citep{Lam2021}. In contrast to passive control strategies, wherein physical elements (e.g. metastructures, plenum windows) are used to disrupt the sound waves, ANC utilises active elements (e.g. microphones, processing units) that drive actuator(s) (e.g. loudspeaker) to generate an "anti-noise" wave that destructively interferes with the impinging noise to attenuate it. Recently, proof-of-principle ``anti-noise'' window systems demonstrated substantial noise mitigation potential on open façade apertures for NV \citep{Lam2020c,Lam2020}. The anti-noise window (ANW) employs sensors (e.g. microphones) outside the window to obtain time-advanced information of the impinging noise, and subsequently computes an equal and opposing anti-noise wave that is reproduced from an array of spatially-optimised loudspeakers, resulting in destructive interference (i.e. acoustic attenuation). 

\subsection{Informational Masking}

Noise control measures for façade openings that preserve NV, with active or passive techniques, is still technically challenging and are effective for a limited range of acoustic frequencies \citep{Lam2021}. Hence, active interference techniques -- an active sound source that projects audio material to "mask" the noise source -- that have been widely employed in office spaces to provide speech privacy could potentially be extended to dwellings \citep{Lenne2020}. Similar to ANC, active interference employs an active sound source to project the masking sounds (``maskers") and would also allow for NV. 

When these maskers overlap spectrotemporally such that the target sound (``noise'') can no longer be audible, ``energetic masking'' occurs \citep{Brungart2001,Culling2017a}. This is akin to the principles in the psychoacoustic masking models employed in audio compression standards \citep{InternationalOrganizationforStandardization1993,Kidd2008}, where only audible sounds are encoded. In contrast, ``informational masking'' (IM) is a broad categorization of phenomena that result in the reduced audibility of noise even in the absence of spectrotemporal overlap with the maskers \citep{Kidd2017}. With the adoption of the soundscape ISO standard \citep{InternationalOrganizationforStandardization2014ISOFramework,InternationalOrganizationforStandardization2018,InternationalOrganizationforStandardization2019}, there is increasing evidence showing that IM or augmentation of outdoor urban noise with biophillic maskers positively impacts affect and health outcomes \citep{Buxton2021,Hong2020h,Leung2017,Coensel2011b,VanRenterghem2020,Jeon2010}.

Owing to the dependency of the soundscape perception on context \citep{InternationalOrganizationforStandardization2014ISOFramework}, however, biophillic maskers that were effective in outdoor urban environments may not be perceived equally in indoor spaces \citep{Torresin2019,Torresin2020IndoorBuildings}. With limited research on biophillic maskers for indoor soundscapes, the suitability and efficacy of IM as an NV-preserving noise mitigation method in indoor spaces still remains an open question  \citep{Hasegawa2021AudiovisualReview}.

\subsection{Human perception in noise control}

Since both ANC and active interference techniques require similar active elements, they have been integrated to form a class of perceptually-driven ANC techniques. However, perceptual ANC systems are usually based on energetic masking principles to shape the residual audio after ANC to achieve desired perceptual objectives \citep{Kajikawa2012c,Jiang2018,Lam2021}. For instance, most of the perceptually-driven ANC systems were designed to meet industrial demand for automobile cabin sound quality \citep{Rees2006AdaptiveSound-profiling,Patel2017ModifiedProfiling,Jiang2018}, and music playback quality in ANC headphones \citep{Belyi2019}. With only a single reported instance of integration of ANC with stream sounds to mitigate snoring noise \citep{Liu2019}, the combination of biophillic maskers with ANC is still underexplored, at least for NV indoor spaces.

Due to the widespread adoption of A-weighted SPL [i.e. \si{\decibelA}] in noise regulations and WHO guidelines, the effectiveness of noise abatement measures is almost always evaluated with \si{\decibelA}-based measures such as insertion loss (IL) and reduction in A-weighted equivalent sound pressure levels (SPL). However, there is growing evidence pointing to the shortcomings of A-weighted SPL in its lack of association with annoyance \citep{Kang2017,Lercher2017CommunityAnalysis}, and its underestimation of low-frequency noise and its potential health effects \citep{AraujoAlves2020a,Baliatsas2016}. It is worth highlighting that suppression of low-frequencies in \si{\decibelA}-based metrics also potentially undermines the perceptual benefit of ANC, which is predominantly effective at mitigating low-frequency noise \citep{Cheer2016ActiveYacht}. Moreover, the overall annoyance perceived in dwellings is modulated by different noise types (e.g. aircraft, traffic, train) and their interactions that are difficult to be captured in \si{\decibelA}-based metrics \citep{Munzel2014CardiovascularExposure,Miedema2004a, Lercher2017CommunityAnalysis}. With the introduction of maskers, an increase in SPL is to be expected, and thus alternative evaluation methodologies that evaluate the overall perception of the acoustic environment, such as the triangulation method in ISO 12913-3, should be adopted \citep{InternationalOrganizationforStandardization2019,Fusaro2022AssessmentPerception}.

\subsection{Research questions}

To address the dearth of research with regards to the perception of ANC and its interaction with biophillic maskers in indoor soundscapes, this study evaluates the perceptual effects of a ANC-based ANW in mitigating typical urban noise and its interaction with a proposed introduction of biophillic maskers. In particular, the following research questions would be addressed:

\begin{enumerate}
  \item[RQ1.] Does the active reduction of low-frequencies in typical urban noise types by an ANW translate to reduced comfort (i.e. perceived annoyance, perceived loudness, perceived affective quality, sentiment) in the context of dwellings?
  \item[RQ2.] In terms of objective performance and comfort perception, what is the effect of IM with representative biophillic maskers on the ANW in mitigating typical urban noise?
  \item[RQ3.] In the context of evaluating novel acoustic solutions to improve indoor soundscape, can perceived acoustic comfort be reliably estimated with only objective parameters?
\end{enumerate}


==> tables/circumplextests.tex <==
\setcounter{table}{2}
\begin{table}[ht]
\begin{minipage}{1\linewidth}
\caption{Summary of circumplex model fitting indexes, where conformity to the recommended threshold is indicated in \textbf{bold}. Abbreviations: CI = Communality Index, CFI = Comparative Fit Index, RMSEA = Root Mean Square Error of Approximation, SRMSR = Standardized Root Mean Squared Residual.} \label{tab:circumplexresults}
\end{minipage}

\begin{tabularx}{1\textwidth}{
>{\raggedright\arraybackslash}p{6cm}%
>{\raggedright\arraybackslash}p{2cm}%
>{\raggedright\arraybackslash}X%
>{\raggedleft\arraybackslash}p{2cm}%
>{\raggedleft\arraybackslash}p{2cm}%
}

\toprule
& &
& AMSS 
& Ambient \\

\midrule\addlinespace[2.5pt] 
\multirow{2}{2cm}{Circular Order}
& CI 
& 
& 0.6806 
& 0.6319 \\ 

& $p$ 
& 
& **0.0032 
& **0.0024 \\

\midrule\addlinespace[2.5pt]
Circulant (Equal communality and angles)
& SSM 
& $\ge$ 0.70
& \textbf{0.7851}
& 0.4028 \\

\midrule\addlinespace[2.5pt]
\multirow[t]{3}{6cm}{Quasi-circumplex} 
& CFI 
& $\ge$ 0.90
& \textbf{0.9530}
& \textbf{0.9340} \\

& RMSEA 
& $\le$ 0.13
& \textbf{0.1190}
& 0.1490 \\

& SRMSR 
& $<$ 0.06
& 0.1010 
& \textbf{0.0410} \\

\midrule\addlinespace[2.5pt]
\multirow[t]{3}{6cm}{Equal angles} 
& CFI 
& $\ge$ 0.90
& 0.6510 
& 0.7750 \\

& RMSEA 
& $\le$ 0.13
& 0.2500 
& 0.2110 \\ 

& SRMSR 
& $<$ 0.06
& 0.2200 
& 0.1560 \\ 

\midrule\addlinespace[2.5pt]
\multirow[t]{3}{6cm}{Equal communality} 
& CFI 
& $\ge$ 0.90
& \textbf{0.9240} 
& \textbf{0.9030} \\

& RMSEA 
& $\le$ 0.13
& \textbf{0.1160} 
& 0.1380 \\

& SRMSR 
& $<$ 0.06
& 0.1270 
& 0.0850 \\ 

\midrule\addlinespace[2.5pt]

\multirow[t]{3}{6cm}{Equal communality and angles} 
& CFI 
& $\ge$ 0.90
& 0.5940 
& 0.5720 \\

& RMSEA 
& $\le$ 0.13
& 0.2270 
& 0.2450 \\ 

& SRMSR 
& $<$ 0.06
& 0.2330 
& 0.2420 \\ 

\bottomrule
\end{tabularx}
\end{table}



==> tables/kstest_piq.tex <==
\setlength{\LTpost}{0mm}
\setcounter{table}{1}
\small
%\footnotesize
\begin{table}[H]

\centering

\begin{minipage}{1\linewidth}
\caption{Summary of exact two-sample Kolmogorov-Smirnov tests to examine the effect of non-acoustic factors (PSS-10, WNSS, WHO-5, baseline annoyance) across each condition (\amss\ and \amb).} \label{tab:kstest_piq}
\end{minipage}

\begin{tabularx}{0.5\linewidth}{
>{\raggedright\arraybackslash}p{5em}%
*{2}{>{\raggedleft\arraybackslash}p{7em}}%
>{\raggedleft\arraybackslash}X}

\toprule
& \textbf{\amb}, N = 32
& \textbf{\amss}, N = 36
& \textbf{p-value} \\

\midrule\addlinespace[2.5pt]

PSS-10 
& 0.51 (0.13) & 0.51 (0.14) & 0.94 \\

INS 
& 0.67 (0.05) & 0.67 (0.06) & 0.72 \\ 

WHO-5 
& 0.59 (0.17) & 0.65 (0.16) & 0.54 \\ 

BA\textsubscript{aircraft} 
& 3.88 (1.41) & 3.97 (1.38) & 0.82 \\ 

BA\textsubscript{mrt} 
& 2.59 (1.29) & 2.14 (1.13) & 0.46 \\ 

BA\textsubscript{consite} 
& 3.59 (1.29) & 3.47 (1.32) & 0.80 \\ 

BA\textsubscript{reno} 
& 3.59 (1.39) & 3.33 (1.31) & 0.59 \\ 

BA\textsubscript{traffic} 
& 3.53 (1.14) & 3.39 (1.27) & 0.90 \\

BA\textsubscript{animals} 
& 1.94 (1.05) & 2.28 (1.14) & 0.28 \\ 

BA\textsubscript{children} 
& 2.66 (1.21) & 2.39 (1.13) & 0.51 \\ 

BA\textsubscript{people} 
& 2.47 (1.05) & 2.22 (0.99) & 0.28 \\ 

BA\textsubscript{others} 
& 2.38 (1.10) & 2.33 (1.26) & 0.83 \\ 

\bottomrule

\end{tabularx}
\end{table}

==> tables/meanpaq.tex <==
\setlength{\LTpost}{0mm}
\begin{table}[ht]
\centering
\caption{Mean responses $\mu$ ($\pm$ standard deviation $\sigma$) of perceptual attributes in the site evaluation questionnaire investigated for the validation study, organized by \textit{site} and \textit{condition}. The scales for all attributes are normalised to the range [$-$1,1]. Percentage changes are computed between the ``Ambient'' and ``AMSS'' conditions as scale changes on the [$-$1,1] range with respect to the ``Ambient'' condition. For instance, a change from $-$0.25 in the ``Ambient'' condition to 0.75 in the ``AMSS'' condition would be reported as a \SI{50}{\percent} change.}
\label{tab:meanpaq}
\def\arraystretch{1.15} %Toggles cell height.

\begin{tabularx}{1.05\linewidth}{lcccccc}
\toprule

\textit{site} & \multicolumn{3}{c}{GFP} & \multicolumn{3}{c}{RTGP} \\
\cline{2-7}
\textit{condition} & Ambient & AMSS & Change (\%) & Ambient & AMSS & Change (\%) \\
\midrule
$\text{DOM}_\text{Noi}$& 0.2500 $\pm$ 0.4399& 0.1528 $\pm$ 0.5045& $-$4.9& 0.6562 $\pm$ 0.3902& 0.5139 $\pm$ 0.4223& $-$7.1 \\
$\text{DOM}_\text{Nat}$& 0.1875 $\pm$ 0.3966& 0.1667 $\pm$ 0.4928& $-$1.0& $-$0.3594 $\pm$ 0.4957& 0.1944 $\pm$ 0.4355& 27.7 \\
$\text{DOM}_\text{Hum}$& $-$0.2500 $\pm$ 0.3810& $-$0.2361 $\pm$ 0.6034& 0.7& $-$0.8594 $\pm$ 0.3416& $-$0.9306 $\pm$ 0.3413& $-$3.6 \\
OQ& 0.1719 $\pm$ 0.4685& 0.1389 $\pm$ 0.3893& $-$1.6& $-$0.1719 $\pm$ 0.5018& 0.0694 $\pm$ 0.5497& 12.1 \\
APPR& $-$0.0156 $\pm$ 0.3911& 0.1528 $\pm$ 0.4443& 8.4& $-$0.3750 $\pm$ 0.4919& 0.0139 $\pm$ 0.5668& 19.4 \\
PLN& $-$0.1719 $\pm$ 0.3503& $-$0.1111 $\pm$ 0.4944& 3.0& 0.3438 $\pm$ 0.4295& 0.1528 $\pm$ 0.5454& $-$9.5 \\
REV& $-$0.3387 $\pm$ 0.4161& $-$0.2500 $\pm$ 0.3744& 4.4& $-$0.5781 $\pm$ 0.4038& $-$0.2639 $\pm$ 0.5276& 15.7 \\
ISOPL& 0.1587 $\pm$ 0.3228& 0.1387 $\pm$ 0.3011& $-$1.0& $-$0.1907 $\pm$ 0.3812& 0.1016 $\pm$ 0.4486& 14.6 \\
ISOEV& 0.0253 $\pm$ 0.2303& 0.0490 $\pm$ 0.2344& 1.2& 0.0553 $\pm$ 0.2392& 0.0789 $\pm$ 0.2599& 1.2 \\
PRSS& $-$0.1215 $\pm$ 0.4088& $-$0.0175 $\pm$ 0.3388& 5.2& $-$0.4126 $\pm$ 0.3799& $-$0.0406 $\pm$ 0.4605& 18.6 \\
PA& $-$0.0719 $\pm$ 0.4252& $-$0.0694 $\pm$ 0.5047& 0.1& $-$0.2125 $\pm$ 0.3782& 0.0694 $\pm$ 0.5879& 14.1 \\
NA& $-$0.8812 $\pm$ 0.1839& $-$0.8778 $\pm$ 0.2344& 0.2& $-$0.7844 $\pm$ 0.2996& $-$0.8278 $\pm$ 0.4340& $-$2.2 \\

\bottomrule
\end{tabularx}
% \begin{minipage}{0.7\linewidth}
% \textsuperscript{\textit{1}}Reported as ``Mean (Standard deviation)''\\
% \textsuperscript{\textit{2}}Wilcoxon rank sum exact test; Wilcoxon rank sum test\\
% \end{minipage}
\end{table}

==> tables/questionnaireIPANAS.tex <==
\begin{sffamily}
\begin{nolinenumbers}
\small%
%\setcounter{table}{1}
\refstepcounter{table} \label{tab:question}
\noindent\textbf{\color{scolor}Table \thetable}\par%
\noindent{I-PANAS-SF}%
% \par\vskip12pt
\end{nolinenumbers}
\small%
\setlength\LTleft{0pt}
\setlength\LTright{0pt}

\begin{longtable}{@{\extracolsep{\fill}}%
>{\raggedright\arraybackslash}p{0.15\textwidth}%
>{\raggedright\arraybackslash}p{0.35\textwidth}%
>{\raggedright\arraybackslash}p{0.2\textwidth}%
>{\raggedright\arraybackslash}p{0.2\textwidth}}

% first head
    \toprule
    Question Category
    & Instructions 
    & Specific Questions
    & Rating Scale\\
    \midrule
\endhead

    \multicolumn{4}{r}{[Continued on next page]} 
\endfoot

    \bottomrule
    
\endlastfoot

    \multirow[t]{10}{=}{I-PANAS-SF}
    & \multirow[t]{10}{=}{This scale consists of a number of words and phrases that describe different feelings and emotions. Read each item and then mark the appropriate answer in the space next to that word. Indicate to what extent you have felt this way in this moment. Use the following scale to record your answers:} 
    & \underline{\hspace{1.5cm}} `active'
    & \multirow[t]{10}{=}{very slightly or not at all--extremely (5-point categorical)}\\ \cline{3-3}

    & & \underline{\hspace{1.5cm}} `attentive' 
    & \\ \cline{3-3} 

    & & \underline{\hspace{1.5cm}} `alert’ 
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}} `determined’ 
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}} `inspired’  
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}} `hostile' 
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}}`ashamed’ 
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}}`upset’ 
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}}`afraid’
    & \\ \cline{3-3}

    & & \underline{\hspace{1.5cm}}`nervous’
    & \\ \cline{3-3}

\end{longtable}
\end{sffamily}
